Greedy Policy Search: A Simple Baseline for Learnable Test-Time Augmentation

Test-time data augmentation$-$averaging the predictions of a machine learning model across multiple augmented samples of data$-$is a widely used technique that improves the predictive performance. While many advanced learnable data augmentation techniques have emerged in recent years, they are focused on the training phase. Such techniques are not necessarily optimal for test-time augmentation and can be outperformed by a policy consisting of simple crops and flips. The primary goal of this paper is to demonstrate that test-time augmentation policies can be successfully learned too. We introduce greedy policy search (GPS), a simple but high-performing method for learning a policy of test-time augmentation. We demonstrate that augmentation policies learned with GPS achieve superior predictive performance on image classification problems, provide better in-domain uncertainty estimation, and improve the robustness to domain shift.

==> instructions.tex <==
% \section{FIRST LEVEL HEADINGS}
% \subsection{SECOND LEVEL HEADING}
% \subsubsection{Third Level Heading}
% \vskip .5pc
% Fourth Level Heading

% Citations within the text should include the author's last name and
% year, e.g., (Cheesman, 1985). Reference style should follow the style
% that you are used to using, as long as the citation style is
% consistent.

% \subsubsection{Footnotes}

% Indicate footnotes with a number\footnote{Sample of the first
% footnote} in the text. Use 8 point type for footnotes.  Place the
% footnotes at the bottom of the page on which they appear.  Precede the
% footnote with a 0.5 point horizontal rule 1~inch (6~picas)
% long.\footnote{Sample of the second footnote}

% \subsubsection{Figures}

% All artwork must be centered, neat, clean, and legible. Figure number
% and caption always appear below the figure.  Leave 2 line spaces
% between the figure and the caption. The figure caption is initial caps
% and each figure numbered consecutively.

% Make sure that the figure caption does not get separated from the
% figure. Leave extra white space at the bottom of the page rather than
% splitting the figure and figure caption.
% \begin{figure}[h]
% \vspace{1in}
% \caption{Sample Figure Caption}
% \end{figure}

% All tables must be centered, neat, clean, and legible. Table number
% and title always appear above the table.  See
% Table~\ref{sample-table}.

% One line space before the table title, one line space after the table
% title, and one line space after the table. The table title must be
% initial caps and each table numbered consecutively.

% \begin{table}[h]
% \caption{Sample Table Title}
% \label{sample-table}
% \begin{center}
% \begin{tabular}{ll}
% \multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION} \\
% \hline \\
% Dendrite         &Input terminal \\
% Axon             &Output terminal \\
% Soma             &Cell body (contains cell nucleus) \\
% \end{tabular}
% \end{center}
% \end{table}

% \subsubsection*{Acknowledgements}
% Use unnumbered third level headings for the acknowledgements title.
% All acknowledgements go at the end of the paper.

% References follow the acknowledgements.  Use unnumbered third level
% heading for the references title.  Any choice of citation style is
% acceptable as long as you are consistent.

